Grad-CAM: Visual Explanations from Deep Networks via Gradient-based Localization

We propose a technique for producing "visual explanations" for decisions from a large class of CNN-based models, making them more transparent. Our approach - Gradient-weighted Class Activation Mapping (Grad-CAM), uses the gradients of any target concept, flowing into the final convolutional layer to produce a coarse localization map highlighting important regions in the image for predicting the concept. Grad-CAM is applicable to a wide variety of CNN model-families: (1) CNNs with fully-connected layers, (2) CNNs used for structured outputs, (3) CNNs used in tasks with multimodal inputs or reinforcement learning, without any architectural changes or re-training. We combine Grad-CAM with fine-grained visualizations to create a high-resolution class-discriminative visualization and apply it to off-the-shelf image classification, captioning, and visual question answering (VQA) models, including ResNet-based architectures. In the context of image classification models, our visualizations (a) lend insights into their failure modes, (b) are robust to adversarial images, (c) outperform previous methods on localization, (d) are more faithful to the underlying model and (e) help achieve generalization by identifying dataset bias. For captioning and VQA, we show that even non-attention based models can localize inputs. We devise a way to identify important neurons through Grad-CAM and combine it with neuron names to provide textual explanations for model decisions. Finally, we design and conduct human studies to measure if Grad-CAM helps users establish appropriate trust in predictions from models and show that Grad-CAM helps untrained users successfully discern a 'stronger' nodel from a 'weaker' one even when both make identical predictions. Our code is available at https://github.com/ramprs/grad-cam/, along with a demo at http://gradcam.cloudcv.org, and a video at youtu.be/COjUB9Izk6E.

==> sections/class_dependence.tex <==

\ijcv{
\subsection{\gcam{} is class-discriminative}
In this section we show why \gcam{} visualizations are class-discriminative.
Recall that $\alpha^k_c$~\eqref{eq:alpha1} can be extracted from any layer of the deep CNN.
Consider a simple cascaded deep CNN for classification having non-linear activation functions given by $\sigma_l(.)$ between layers $l$ and $(l+1)$. The scores corresponding to classes can be expressed as $\mathbf{y} = W_f^TA_f$ where $W_f$ and $A_f$ correspond to the final layer weights and activations respectively. 
Let $o_c$ be the incoming gradient from the loss layer. Note that $o_c$ is a one-hot vector with $1$ at the dimension corresponding to class $c$ and $0$ everywhere else.
With this, $\alpha_c^k$ of \gcam{} can be written in terms of $\mathbf{y}$ and $o_c$ as,
\begin{ceqn}
\begin{equation}
\alpha_c^k = \frac{1}{Z} \sum_i \sum_j \frac{\partial (\mathbf{y}\circ o_c)}{\partial A^k_{ij}}
\end{equation}
\end{ceqn}
where $\circ$ denotes the elementwise product.
Since $o_c$ is a constant, $\frac{\partial (o_c)}{\partial A^k_{ij}} = 0$. Thus we obtain,
\begin{ceqn}
\begin{equation}
\alpha_c^k = (\frac{1}{Z} \sum_i \sum_j \frac{\partial \mathbf{y}}{\partial A^k_{ij}})\circ o_c
\end{equation}
\end{ceqn}
Now, recall that due to chain rule, this gradient expression above can be rewritten as a product of partial derivatives along the computation path:
\begin{ceqn}
\begin{equation}
 \alpha_c^k = (\frac{1}{Z} \sum_{i,j} \frac{\partial \mathbf{y}}{\partial A_{f-1}} \frac{\partial A_{f-1}}{\partial \sigma_{A_{f-1}}} \frac{\partial \sigma_{A_{f-1}}}{\partial A_{f-2}}\frac{\partial A_{f-2}}{\partial \sigma_{A_{f-2}}}...)\circ o_c
\end{equation}
\end{ceqn}
Recall that $\frac{\partial (y)}{\partial A_{f-1}}$ is $W_f$, and similarly $\frac{\partial \sigma_{A_{l}}}{\partial A_{l-1}}$ is $W_{l}$.
The gradients \wrt activation functions results in diagonal matrices, $D_{\sigma_l}$. For networks with ReLU activations, the entries in the diagonal matrices are either 1 or 0 depending on whether the forward activations at that location is positive or negative, respectively. By substituting we get,
\begin{ceqn}
\begin{equation}
 \alpha_c^k = (\frac{1}{Z} \sum_{i,j} W_f D_{\sigma_{f-1}} W_{f-1} D_{\sigma_{f-2}}...)\circ o_c
\end{equation}
\end{ceqn}
The above expression can be reduced to,
\begin{ceqn}
\begin{equation}
 \alpha_c^k = (\frac{1}{Z} \sum_{i,j} \prod_{l=f}^L D_{\sigma_{l-1}} W_{l}) \circ o_c
\end{equation}
\end{ceqn}
where $W_{l}$ denote the weights connecting layers $(l-1)$ and $l$, and $l = \{ f, f-1, ..., L \}$.
Therefore, $\alpha_c^k$ explicitly captures the dynamics of the pathways leading from $L$ (last convolutional layer) to the target class score, $y_c$ in the network.
This makes neuron-importance weights, $\alpha_c^k$ and by extension \gcam{} class-discriminative.}












==> sections/neg_exp.tex <==
\section{Counterfactual Explanations}
We propose a new explanation modality -- counterfactual explanations.
Using a slight modification to \gcam{}, we can obtain explanations
that highlight support for regions that would make the network change its prediction.
As a consequence, removing concepts occurring in those regions would make the
model more confident about its prediction.

Specifically, we negate the gradient of $y^c$ (score for class $c$) with respect to feature maps $A$ of a convolutional layer.
Thus the importance weights $\alpha{}_{k}^{c}$ now become
\begin{ceqn}
\begin{equation} \label{eq:alpha_neg}
    \alpha{}_{k}^c =
    \overbrace{
        \frac{1}{Z}\sum_{i}\sum_{j}
    }^{\text{global average pooling}}
    \hspace{-17pt}
    \underbrace{
        \vphantom{\sum_{i}\sum_{j}} -\frac{\partial y^c}{\partial A_{ij}^{k}}
    }_{\text{Negative gradients}}
\end{equation}
\end{ceqn}
As in \eqref{eq:gcam}, we take a weighted sum of the forward activation maps, $A$, with weights $\alpha{}_{k}^c$, and follow it by a ReLU to obtain counterfactual explanations as shown in \reffig{fig:negexp}.

\begin{figure}[ht!]
    \centering \begin{subfigure}[t]{0.158\textwidth} \centering
        \includegraphics[width=\textwidth]{figures/teaser/original.jpg}
        \caption{\scriptsize{Original Image}}
	\end{subfigure}
	\begin{subfigure}[t]{0.158\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/cat_neg_exp.jpg}
        \caption{\scriptsize{Cat Counterfactual exp}}
		\label{fig:neg_exp_cat}
	\end{subfigure}
    \centering
	\begin{subfigure}[t]{0.158\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/dog_neg_exp.jpg}
        \caption{\ijcv{\scriptsize{\hspace{-1pt}Dog Counterfactual exp}}}%
		\label{fig:neg_exp_dog}
	\end{subfigure}
    \vspace{10pt}
    \caption{Counterfactual Explanations with \gcam{}}
    \label{fig:negexp}
\end{figure}


==> sections/sup_bias.tex <==
\vspace{-15pt}
\section{Identifying and removing bias in datasets}\label{sec:sup_bias}

In this section we provide qualitative examples showing the explanations from the two models trained for distinguishing doctors from nurses- model1 which was trained on images (with an inherent bias) from a popular search engine, and model2 which was trained on a more balanced set of images from the same search engine.

As shown in \reffig{fig:sup_bias}, \gcam{} visualizations of the model (model1) predictions show that
the model had learned to look at the person's face / hairstyle to distinguish nurses from doctors, thus learning a gender stereotype.

Using the insights gained from the \gcam{} visualizations, we balanced the dataset and retrained the model. The new model, model2 not only generalizes well to a balanced test set, it also looks at the right regions, as can be seen in \reffig{fig:sup_bias}.
\begin{figure}[ht!]
\vspace{20pt}
  \begin{center}
    \begin{subfigure}[b]{0.32\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{figures/71_orig_balanced.jpg}
		\caption{\tiny{Original Image}}
        \vspace{10pt}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{figures/71_gcam_incorr_unbalanced.jpg}
		\caption{\tiny{\gcam{} for biased model}}
        \vspace{10pt}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{figures/71_gcam_corr_balanced.jpg}
		\caption{\tiny{\gcam{} for unbiased model}}
        \vspace{10pt}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{figures/teaser/25_orig_balanced.jpg}
		\caption{\tiny{Original image}}
        \vspace{10pt}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{figures/teaser/25_gcam_incorr_unbalanced.jpg}
		\caption{\tiny{\gcam{} for biased model}}
        \vspace{10pt}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{figures/teaser/25_gcam_corr_balanced.jpg}
		\caption{\tiny{\gcam{} for unbiased model}}
        \vspace{10pt}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{figures/teaser/60_orig_balanced.jpg}
		\caption{\tiny{Original Image}}
        \vspace{10pt}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{figures/teaser/60_gcam_incorr_unbalanced.jpg}
		\caption{\tiny{\gcam{} for biased model}}
        \vspace{10pt}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{figures/teaser/60_gcam_corr_balanced.jpg}
		\caption{\tiny{\gcam{} for unbiased model}}
        \vspace{10pt}
    \end{subfigure}
    \vspace{10pt}
	\caption{\ijcv{\gcam{} explanations for model1 and model2. 
    In all the 3 examples we see that the biased model was looking at the face of the person to predict `nurse' incorrectly, whereas the unbiased model looks at the stethoscope and the white coat to correctly predict `doctor'.}
    }
    \label{fig:sup_bias}
    \end{center}
    \vspace{-15pt}
\end{figure}

==> sections/sup_gcam_generalization.tex <==
\section*{Appendix I: \gcam{} as generalization of CAM}\label{sec:sup_generalization}

In this section we formally prove that \gcam{} is a generalization of CAM, as mentioned in Section 3 in the main paper.

Recall that the CAM architecture consists of fully-covolutional CNNs, followed by global average pooling, and linear classification layer with softmax.

Let the final convolutional layer produce $K$ feature maps $A^k$, with each element indexed by $i,j$. 
So $A_{ij}^k$ refers to the activation at location $(i,j)$ of the feature map $A^k$.

CAM computes a global average pooling (GAP) on $A_{ij}^k$. Let us define $F^k$ to be the global average pooled output,

So,
\begin{equation}\label{eq:cam_gap} 
    F^{k} = \frac{1}{Z} \sum_{i} \sum_{j} A_{ij}^k
\end{equation}

CAM computes the final scores by,
\begin{equation}\label{eq:cam_scores}
    Y^c = \sum_{k} w_{k}^c \cdot F^{k}
\end{equation}
where $w_{k}^c$ is the weight connecting the $k^{th}$ feature map with the $c^{th}$ class. 

Taking the gradient of the score for class c ($Y^c$)  with respect to the feature map $F^k$ we get,
\begin{equation}\label{eq:cam_grad}
    \qquad \text{(From Chain Rule)}\\
    \frac{\partial Y^c}{\partial F^k} = \frac{\frac{\partial Y^c}{\partial A_{ij}^k}}{\frac{\partial F^k}{\partial A_{ij}^k}}
\end{equation}

Taking partial derivative of  \eqref{eq:cam_gap} \wrt $A_{ij}^k$, we can see that $\frac{\del F^k}{\del A^k_{ij}} = \frac{1}{Z}$. Substituting this in \eqref{eq:cam_grad}, we get,

\begin{equation}
    \frac{\partial Y^c}{\partial F^k} = \frac{\partial Y^c}{\partial A_{ij}^k} \cdot Z\\
\end{equation}

From \eqref{eq:cam_scores} we get that, $ \frac{\partial Y^c}{\partial F^k} = w_{k}^c$. Hence,

\begin{equation}\label{eq:cam_weights}
    w_{k}^c = Z \cdot \frac{\partial Y^c}{\partial A_{ij}^k}\\
\end{equation}

Now, we can sum both sides of this expression in (5) over all pixels $(i,j)$ to get: 

\begin{align}
    \sum_i \sum_j w^c_k  = \sum_i \sum_j Z \cdot \frac{\del Y^c}{\del A^k_{ij} }, \quad \text{which can be rewritten as} \\ 
    Z w^c_k  = Z \sum_i \sum_j \frac{\del Y^c}{\del A^k_{ij} } \quad \text{(Since $Z$ and $w^c_k$ do not depend on $(i,j)$)}
\end{align}

Note that $Z$ is the number of pixels in the feature map (or $Z = \sum_i \sum_j 1 $). 
Thus, we can re-order terms and see that:

\begin{align}
    w^c_k  &= \sum_i \sum_j \frac{\del Y^c}{\del A^k_{ij} }\\
\end{align}

We can see that up to a proportionality constant ($1/Z$) that is normalized out during visualization, the expression for $w^c_k$ is identical to $\alpha^c_k$ used by \gcam{} (as described in the main paper). 


Thus \gcam{} is a generalization of CAM to arbitrary CNN-based architectures, while maintaining the computational efficiency of CAM.



==> sections/sup_intro.tex <==
\section{Introduction}

In \secref{sec:sup_generalization}, we derive that \gcam{} is a generalization of CAM to \emph{any} CNN-based architecture, and hence doesn't require any architectural change or retraining. 
In \secref{sec:sup_experiments} we provide more visual explanations for image classification (VGG-16), image captioning (Neuraltalk2), and Visual Question Answering (VQA). For image captioning and VQA, our visualizations (\gcam{}, and \cgb{}) expose the somewhat surprising insight that common CNN+LSTM
models can often be good at localizing discriminative input image regions despite note being trained on grounded image-text pairs.
In \secref{sec:sup_ablation}, we explore and validate our design choices for computing \gcam{} visualizations. 
In \secref{sec:sup_localization}, we compare the localization ability of \gcam{} with previous approaches in the context of image classification.
In \secref{sec:sup_segmentation}, we show qualitative results by using weak-localization cues from \gcam{} as a seed for SEC~\cite{seed_eccv16}.
In \secref{sec:sup_comparison}, we provide qualitative examples comparing \gcam{} with CAM and c-MWP on two image classification datasets, PASCAL and COCO. We find that our visualizations are superior, while being faster to compute and while being possible to visualize a  \emph{wide variety of CNN-based models, including but not limited to, CNNs with fully-connected layers, CNNs stacked with Recurrent Neural Networks (RNNs), ResNets \etc}.




==> sections/sup_localization.tex <==
\section{Weakly-supervised Localization}\label{sec:sup_localization}
In this section, we compare the localization capability of \gcam{} with previous approaches in the context of image classification.

Following ILSVRC evaluation, we report both top-1 and top-5 localization \rp{error} on ILSVRC-15 validation set in \reftab{table:locres}. 

As can be seen from the table, \gcam{} localizations are significantly better than competing approaches such as c-MWP~\cite{zhang2016top} and Backprop~\cite{simonyan_arxiv13}. We also find that CAM slighly outperforms \gcam{}, but it requires an architectural change, and hence re-training.

\vspace{-10pt}
\begin{table}[h!]
\centering
    \resizebox{0.98\columnwidth}{!}{
        \begin{tabular}{c c c c c}\toprule
            \textbf{Method} & \textbf{Top-1 loc error} & \textbf{Top-5 loc error} & \textbf{Top-1 cls error} & \textbf{Top-5 cls error} \\
            \midrule

            Backprop on VGG-16~\cite{simonyan_arxiv13}  & 61.12 & 51.46 & 30.64 & 11.03        \\
            c-MWP on VGG-16~\cite{zhang2016top}         & 70.92 & 63.04 & 30.64 & 11.03        \\
            \gcam{} on VGG-16                           & 57.80 & 48.03 & 30.64 & 11.03        \\
            \midrule
            VGG-16-GAP~\cite{zhou_cvpr16}               & 57.20 & 45.14 & 33.40 & 12.20        \\
            \bottomrule
        \end{tabular}
    }
    \vspace{-6pt}
    \caption{Classification and Localization results on ILSVRC-15 val.
    \gcam{} outperforms~\cite{simonyan_arxiv13} and c-MWP \cite{zhang2016top} by a significant margin.} 
    \label{table:locres}
    \vspace{-10pt}
\end{table}



==> sections/sup_segmentation.tex <==
\vspace{-20pt}
\section{Weakly-supervised segmentation}\label{sec:sup_segmentation}

In this section we provide more qualitative examples for weakly-supervised segmentation using \gcam{} as seed for SEC (\cite{seed_eccv16}).



The last row shows 2 failure cases. In the bottom left image, the clothes of the 2 person weren't highlighted correctly. This could be because the most discriminative parts are their faces, and hence \gcam{} maps only highlights those. This results in a segmentation that only highlights the faces of the 2 people. 
In the bottom right image, the bicycles, being extremely thin aren't highlighed. This could be because the resolution of the \gcam{} maps are low ($14 \times 14$) which makes it difficult to capture thin areas.

\begin{figure*}[htp]
 \centering
 \includegraphics[width=1\linewidth]{figures/gcam_segmentation.jpg}
 \vspace{5pt}
 \caption{PASCAL VOC 2012 Segmentation results with \gcam{} as seed for SEC~\cite{seed_eccv16}.}
 \label{fig:segmentation}
\end{figure*}


==> updates.tex <==
Dear Editors and Reviewers,
\vspace{5pt}

The submitted manuscript is an extended version of our ICCV 2017 paper ``Grad-CAM: Visual Explanations for Deep Networks via Gradient-based Localization''.
The major extensions over the conference version are listed below:
\begin{enumerate}


\item \textbf{Generating Textual explanations using \gcam{} and named neurons:} In \refsec{sec:text_exp}, we use the neuron-importance weights $\alpha{}$ and combine them with neuron names from \cite{netdissect} to obtain text-based explanations for model decisions.
\vspace{10pt}

\item \textbf{Using \gcam{} for weakly-supervised segmentation:} In \refsec{sec:segmentation}, we use the low-resolution heatmap provided by \gcam{} as weak-supervision to train a segmentation model using the Seed, Expand and Constrain (SEC) loss introduced in \cite{seed_eccv16}.
 \vspace{10pt}

\item \textbf{Evaluating \gcam{} through pointing experiment:} In \refsec{sec:pointing_game}, we evaluate \gcam{} explanations using a modified version of the evaluation technique proposed in ~\cite{zhang2016top} which measures both precision and recall.
 \vspace{10pt}
 
 \item
\textbf{\gcam{} as a generalization to CAM:} In \refsec{sec:generalization},
we prove \gcam{} generalizes Class Activation Mapping (CAM)~\cite{zhou_cvpr16}
to \emph{any} CNN-based architecture and thus does not require any architectural
change or retraining.
 \vspace{10pt}



\item \textbf{Ablation studies:} In \refsec{sec:ablation}, we perform several ablation studies to explore and validate our design choices for computing \gcam{} visualizations. This includes visualizing different layers in the network, understanding importance of ReLU in \eqref{eq:gcam}, analyzing different types of gradients (for ReLU backward pass), and different gradient pooling strategies.
 \vspace{10pt}

 \item \textbf{Robustness to adversarial examples:} In \refsec{sec:adversarial_noise}, we demonstrate the robustness of \gcam{} by synthesizing adversarial examples (so that the model predicts a non-existent class) and computing \gcam{} for the original (existent) category. We find that \gcam{} can still localize the original class even if the prediction of the original class is suppressed.%
 \vspace{10pt}

 \item \textbf{Qualitative results for `Identifying and removing dataset bias' experiment}: In our ICCV '17 paper, we showed a use-case of \gcam{} to identify and remove biases in datasets. We provide more details of the bias experiment in \secref{sec:sup_bias}. Moreover we provide \gcam{} explanations for the models trained with and without biased datasets and show that the latter model not only generalizes better, but also learns to look at the right regions when making decisions.
  \vspace{10pt}

\item \textbf{Counterfactual explanations using \gcam{}:} We introduce a new explanation modality - Counterfactual
explanations, which we obtain through a slight modification to Grad-CAM. Counterfactual explanations highlight the regions that would make the network change
its decision, \ie the regions in the image that are most confusing for the target class.
 \vspace{10pt}

\item \textbf{More qualitative examples:} We provide more qualitative results showing \gcam{} and \cgb{} visualizations for image classification and other vision and language tasks such as, image captioning, and visual question answering (VQA).
 \vspace{10pt}

\item \textbf{Qualitative comparison to existing visualization techniques:} We compare with existing visualization techniques -- CAM and c-MWP, on PASCAL and COCO, where we find our visualizations
to be superior and faster to compute.
 \vspace{10pt}

\item \textbf{Grad-CAM for ResNet architectures}: We show \gcam{} visualizations for a 200-layer ResNet model introduced in \cite{he_cvpr15}, and analyze how the localization ability of \gcam{} changes as we visualize different residual blocks.


\end{enumerate}
\vspace{15pt}

We look forward to comments and feedback from the editors and reviewers.

Sincerely,\\
The authors

